Master Integrals For Massless Two-Loop Vertex Diagrams With Three Offshell Legs

We compute the master integrals for massless two-loop vertex graphs with three off-shell legs. These master integrals are relevant for the QCD corrections to H to V*V* (where V = W, Z) and for two-loop studies of the triple gluon (and quark-gluon) vertex. We employ the differential equation technique to provide series expansions in epsilon for the various master integrals. The results are analytic and contain a new class of two-dimensional harmonic polylogarithms.

==> E12a.tex <==
\frac{-633 - 19\,{\pi }^2 + 60\,\zeta_3}{6}
\\&
+\frac{-5\,{\pi }^2 - 6\,\zeta_3}{12}\,G(0;0,y)\\&
+\frac{5\,{\pi }^2 + 6\,\zeta_3}{12}\,G(0;x,y)\\&
+\frac{5\,{\pi }^2 + 6\,\zeta_3}{12}\,G(\lambda ;0,y)\\&
+\frac{\left( -1 + x + y \right) \,\left( 5\,{\pi }^2 + 6\,\zeta_3 \right) }{12\,\lambda}\,G(\lambda ;x,y)\\&
+\frac{\left( 1 - y \right) \,\left( 5\,{\pi }^2 + 6\,\zeta_3 \right) }{12}\,G(x\lambda ;0,y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right) \,\left( 5\,{\pi }^2 + 6\,\zeta_3 \right)  \right) }{12\,\lambda}\,G(x\lambda ;x,y)\\&
+\frac{-{\pi }^2}{24}\,G(0,0;0,y)\\&
+\frac{-{\pi }^2}{24}\,G(0,0;x,y)\\&
+\frac{-{\pi }^2}{24}\,G(0,\lambda ;0,y)\\&
+\frac{-\left( {\pi }^2\,\left( -1 + x + y \right)  \right) }{8\,\lambda}\,G(0,\lambda ;x,y)\\&
+\frac{{\pi }^2\,\left( -1 + y \right) }{24}\,G(0,x\lambda ;0,y)\\&
+\frac{{\pi }^2\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{8\,\lambda}\,G(0,x\lambda ;x,y)\\&
+(19 + \frac{{\pi }^2}{24})\,G(\lambda ,0;0,y)\\&
+\frac{-\left( \left( -456 + {\pi }^2 \right) \,\left( -1 + x + y \right)  \right) }{24\,\lambda}\,G(\lambda ,0;x,y)\\&
+\frac{{\pi }^2}{24}\,G(\lambda ,\lambda ;0,y)\\&
+\frac{-{\pi }^2}{8}\,G(\lambda ,\lambda ;x,y)\\&
+\frac{-\left( {\pi }^2\,\left( -1 + y \right)  \right) }{24}\,G(\lambda ,x\lambda ;0,y)\\&
+\frac{{\pi }^2\,\left( -1 + y \right) }{8}\,G(\lambda ,x\lambda ;x,y)\\&
+\frac{-{\pi }^2}{12}\,G(x_0,\lambda ;0,y)\\&
+\frac{-\left( {\pi }^2\,\left( -1 + x + y \right)  \right) }{12\,\lambda}\,G(x_0,\lambda ;x,y)\\&
+\frac{{\pi }^2\,\left( -1 + y \right) }{12}\,G(x_0,x\lambda ;0,y)\\&
+\frac{{\pi }^2\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{12\,\lambda}\,G(x_0,x\lambda ;x,y)\\&
+\frac{-{\pi }^2}{12}\,G(x_1,\lambda ;0,y)\\&
+\frac{-\left( {\pi }^2\,\left( -1 + x + y \right)  \right) }{12\,\lambda}\,G(x_1,\lambda ;x,y)\\&
+\frac{{\pi }^2\,\left( -1 + y \right) }{12}\,G(x_1,x\lambda ;0,y)\\&
+\frac{{\pi }^2\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{12\,\lambda}\,G(x_1,x\lambda ;x,y)\\&
+\frac{-\left( {\pi }^2\,\left( -1 + y \right)  \right) }{24}\,G(x\lambda ,0;0,y)\\&
+\frac{{\pi }^2\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{24\,\lambda}\,G(x\lambda ,0;x,y)\\&
+\frac{-\left( {\pi }^2\,\left( -1 + y \right)  \right) }{24}\,G(x\lambda ,\lambda ;0,y)\\&
+\frac{{\pi }^2\,\left( -1 + y \right) }{8}\,G(x\lambda ,\lambda ;x,y)\\&
+\frac{{\pi }^2\,{\left( -1 + y \right) }^2}{24}\,G(x\lambda ,x\lambda ;0,y)\\&
+\frac{-\left( {\pi }^2\,{\left( -1 + y \right) }^2 \right) }{8}\,G(x\lambda ,x\lambda ;x,y)\\&
-5\,G(0,\lambda ,0;0,y)\\&
+\frac{-15\,\left( -1 + x + y \right) }{2\,\lambda}\,G(0,\lambda ,0;x,y)\\&
-5\,G(\lambda ,0,0;0,y)\\&
+\frac{-10\,\left( -1 + x + y \right) }{\lambda}\,G(\lambda ,0,0;x,y)\\&
-\left( \frac{5}{2} \right) \,G(\lambda ,0,\lambda ;0,y)\\&
+\frac{5\,\left( -1 + y \right) }{2}\,G(\lambda ,0,x\lambda ;0,y)\\&
+\frac{5}{2}\,G(\lambda ,\lambda ,0;0,y)\\&
-\left( \frac{15}{2} \right) \,G(\lambda ,\lambda ,0;x,y)\\&
+\frac{5\,\left( -1 + y \right) }{2}\,G(\lambda ,x\lambda ,0;0,y)\\&
-5\,G(x_0,\lambda ,0;0,y)\\&
+\frac{-5\,\left( -1 + x + y \right) }{\lambda}\,G(x_0,\lambda ,0;x,y)\\&
-5\,G(x_1,\lambda ,0;0,y)\\&
+\frac{-5\,\left( -1 + x + y \right) }{\lambda}\,G(x_1,\lambda ,0;x,y)\\&
+(5 - 5\,y)\,G(x\lambda ,\lambda ,0;0,y)\\&
+\frac{15\,\left( -1 + y \right) }{2}\,G(x\lambda ,\lambda ,0;x,y)\\&
+\frac{3}{4}\,G(0,0,\lambda ,0;0,y)\\&
+\frac{9\,\left( -1 + x + y \right) }{4\,\lambda}\,G(0,0,\lambda ,0;x,y)\\&
+\frac{1}{2}\,G(0,\lambda ,0,0;0,y)\\&
+\frac{3\,\left( -1 + x + y \right) }{\lambda}\,G(0,\lambda ,0,0;x,y)\\&
+\frac{3}{4}\,G(0,\lambda ,0,\lambda ;0,y)\\&
+\frac{-3\,\left( -1 + y \right) }{4}\,G(0,\lambda ,0,x\lambda ;0,y)\\&
+\frac{3}{2}\,G(0,\lambda ,\lambda ,0;0,y)\\&
+\frac{3}{4}\,G(0,\lambda ,\lambda ,0;x,y)\\&
+\frac{-3\,\left( -1 + y \right) }{4}\,G(0,\lambda ,x\lambda ,0;0,y)\\&
+G(0,x_0,\lambda ,0;0,y)\\&
+\frac{3\,\left( -1 + x + y \right) }{2\,\lambda}\,G(0,x_0,\lambda ,0;x,y)\\&
+G(0,x_1,\lambda ,0;0,y)\\&
+\frac{3\,\left( -1 + x + y \right) }{2\,\lambda}\,G(0,x_1,\lambda ,0;x,y)\\&
+\frac{-3\,\left( -1 + y \right) }{4}\,G(0,x\lambda ,\lambda ,0;0,y)\\&
+\frac{-3\,\left( -1 + y \right) }{4}\,G(0,x\lambda ,\lambda ,0;x,y)\\&
+G(\lambda ,0,0,0;0,y)\\&
+\frac{4\,\left( -1 + x + y \right) }{\lambda}\,G(\lambda ,0,0,0;x,y)\\&
+G(\lambda ,0,0,\lambda ;0,y)\\&
+(1 - y)\,G(\lambda ,0,0,x\lambda ;0,y)\\&
+\frac{1}{4}\,G(\lambda ,0,\lambda ,0;0,y)\\&
+\frac{9}{4}\,G(\lambda ,0,\lambda ,0;x,y)\\&
+(1 - y)\,G(\lambda ,0,x\lambda ,0;0,y)\\&
+\frac{1}{2}\,G(\lambda ,\lambda ,0,0;0,y)\\&
+3\,G(\lambda ,\lambda ,0,0;x,y)\\&
-\left( \frac{3}{4} \right) \,G(\lambda ,\lambda ,0,\lambda ;0,y)\\&
+\frac{3\,\left( -1 + y \right) }{4}\,G(\lambda ,\lambda ,0,x\lambda ;0,y)\\&
-\left( \frac{3}{2} \right) \,G(\lambda ,\lambda ,\lambda ,0;0,y)\\&
+\frac{3\,\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ,\lambda ,\lambda ,0;x,y)\\&
+\frac{3\,\left( -1 + y \right) }{4}\,G(\lambda ,\lambda ,x\lambda ,0;0,y)\\&
-G(\lambda ,x_0,\lambda ,0;0,y)\\&
+\frac{3}{2}\,G(\lambda ,x_0,\lambda ,0;x,y)\\&
-G(\lambda ,x_1,\lambda ,0;0,y)\\&
+\frac{3}{2}\,G(\lambda ,x_1,\lambda ,0;x,y)\\&
+(1 - y)\,G(\lambda ,x\lambda ,0,0;0,y)\\&
+\frac{3\,\left( -1 + y \right) }{4}\,G(\lambda ,x\lambda ,\lambda ,0;0,y)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ,x\lambda ,\lambda ,0;x,y)\\&
+G(x_0,0,\lambda ,0;0,y)\\&
+\frac{3\,\left( -1 + x + y \right) }{2\,\lambda}\,G(x_0,0,\lambda ,0;x,y)\\&
+G(x_0,\lambda ,0,0;0,y)\\&
+\frac{2\,\left( -1 + x + y \right) }{\lambda}\,G(x_0,\lambda ,0,0;x,y)\\&
+\frac{1}{2}\,G(x_0,\lambda ,0,\lambda ;0,y)\\&
+\frac{1 - y}{2}\,G(x_0,\lambda ,0,x\lambda ;0,y)\\&
+G(x_0,\lambda ,\lambda ,0;0,y)\\&
+\frac{1 - y}{2}\,G(x_0,\lambda ,x\lambda ,0;0,y)\\&
+G(x_0,x_0,\lambda ,0;0,y)\\&
+\frac{-1 + x + y}{\lambda}\,G(x_0,x_0,\lambda ,0;x,y)\\&
+G(x_0,x_1,\lambda ,0;0,y)\\&
+\frac{-1 + x + y}{\lambda}\,G(x_0,x_1,\lambda ,0;x,y)\\&
+\frac{1 - y}{2}\,G(x_0,x\lambda ,\lambda ,0;0,y)\\&
+G(x_1,0,\lambda ,0;0,y)\\&
+\frac{3\,\left( -1 + x + y \right) }{2\,\lambda}\,G(x_1,0,\lambda ,0;x,y)\\&
+G(x_1,\lambda ,0,0;0,y)\\&
+\frac{2\,\left( -1 + x + y \right) }{\lambda}\,G(x_1,\lambda ,0,0;x,y)\\&
+\frac{1}{2}\,G(x_1,\lambda ,0,\lambda ;0,y)\\&
+\frac{1 - y}{2}\,G(x_1,\lambda ,0,x\lambda ;0,y)\\&
+G(x_1,\lambda ,\lambda ,0;0,y)\\&
+\frac{1 - y}{2}\,G(x_1,\lambda ,x\lambda ,0;0,y)\\&
+G(x_1,x_0,\lambda ,0;0,y)\\&
+\frac{-1 + x + y}{\lambda}\,G(x_1,x_0,\lambda ,0;x,y)\\&
+G(x_1,x_1,\lambda ,0;0,y)\\&
+\frac{-1 + x + y}{\lambda}\,G(x_1,x_1,\lambda ,0;x,y)\\&
+\frac{1 - y}{2}\,G(x_1,x\lambda ,\lambda ,0;0,y)\\&
+\frac{3\,\left( -1 + y \right) }{4}\,G(x\lambda ,0,\lambda ,0;0,y)\\&
+\frac{-9\,\left( -1 + y \right) }{4}\,G(x\lambda ,0,\lambda ,0;x,y)\\&
+\frac{-1 + y}{2}\,G(x\lambda ,\lambda ,0,0;0,y)\\&
+(3 - 3\,y)\,G(x\lambda ,\lambda ,0,0;x,y)\\&
+\frac{3\,\left( -1 + y \right) }{4}\,G(x\lambda ,\lambda ,0,\lambda ;0,y)\\&
+\frac{-3\,{\left( -1 + y \right) }^2}{4}\,G(x\lambda ,\lambda ,0,x\lambda ;0,y)\\&
+\frac{3\,\left( -1 + y \right) }{2}\,G(x\lambda ,\lambda ,\lambda ,0;0,y)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ,\lambda ,\lambda ,0;x,y)\\&
+\frac{-3\,{\left( -1 + y \right) }^2}{4}\,G(x\lambda ,\lambda ,x\lambda ,0;0,y)\\&
+(-1 + y)\,G(x\lambda ,x_0,\lambda ,0;0,y)\\&
+\frac{-3\,\left( -1 + y \right) }{2}\,G(x\lambda ,x_0,\lambda ,0;x,y)\\&
+(-1 + y)\,G(x\lambda ,x_1,\lambda ,0;0,y)\\&
+\frac{-3\,\left( -1 + y \right) }{2}\,G(x\lambda ,x_1,\lambda ,0;x,y)\\&
+\frac{-3\,{\left( -1 + y \right) }^2}{4}\,G(x\lambda ,x\lambda ,\lambda ,0;0,y)\\&
+\frac{3\,{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ,x\lambda ,\lambda ,0;x,y)\\&
+(\frac{-5\,{\pi }^2}{6} - \zeta_3)\,H(1;y)\\&
-19\,H(1,0;y)\\&
+\frac{-{\pi }^2}{6}\,H(1,1;y)\\&
+10\,H(1,0,0;y)\\&
-5\,H(1,1,0;y)\\&
-4\,H(1,0,0,0;y)\\&
+2\,H(1,1,0,0;y)\\&
-H(1,1,1,0;y)\\&
+\frac{{\pi }^2}{24}\,G(0;0,y)\,G(0;x,y)\\&
+\frac{{\pi }^2\,\left( -1 + x + y \right) }{24\,\lambda}\,G(0;0,y)\,G(\lambda ;x,y)\\&
+\frac{-\left( {\pi }^2\,\left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{24\,\lambda}\,G(0;0,y)\,G(x\lambda ;x,y)\\&
-\left( \frac{19}{2} \right) \,G(0;0,y)\,H(0;y)\\&
+\frac{-{\pi }^2}{12}\,G(0;0,y)\,H(1;y)\\&
+5\,G(0;0,y)\,H(0,0;y)\\&
-\left( \frac{5}{2} \right) \,G(0;0,y)\,H(1,0;y)\\&
-2\,G(0;0,y)\,H(0,0,0;y)\\&
+G(0;0,y)\,H(1,0,0;y)\\&
-\left( \frac{1}{2} \right) \,G(0;0,y)\,H(1,1,0;y)\\&
+\frac{-{\pi }^2}{24}\,G(0;x,y)\,G(\lambda ;0,y)\\&
+\frac{{\pi }^2\,\left( -1 + y \right) }{24}\,G(0;x,y)\,G(x\lambda ;0,y)\\&
-\left( \frac{5}{2} \right) \,G(0;x,y)\,G(\lambda ,0;0,y)\\&
+\frac{1}{2}\,G(0;x,y)\,G(0,\lambda ,0;0,y)\\&
+\frac{1}{2}\,G(0;x,y)\,G(\lambda ,0,0;0,y)\\&
+\frac{1}{4}\,G(0;x,y)\,G(\lambda ,0,\lambda ;0,y)\\&
+\frac{1 - y}{4}\,G(0;x,y)\,G(\lambda ,0,x\lambda ;0,y)\\&
-\left( \frac{1}{4} \right) \,G(0;x,y)\,G(\lambda ,\lambda ,0;0,y)\\&
+\frac{1 - y}{4}\,G(0;x,y)\,G(\lambda ,x\lambda ,0;0,y)\\&
+\frac{1}{2}\,G(0;x,y)\,G(x_0,\lambda ,0;0,y)\\&
+\frac{1}{2}\,G(0;x,y)\,G(x_1,\lambda ,0;0,y)\\&
+\frac{-1 + y}{2}\,G(0;x,y)\,G(x\lambda ,\lambda ,0;0,y)\\&
+\frac{19}{2}\,G(0;x,y)\,H(0;y)\\&
+\frac{{\pi }^2}{12}\,G(0;x,y)\,H(1;y)\\&
-5\,G(0;x,y)\,H(0,0;y)\\&
+\frac{5}{2}\,G(0;x,y)\,H(1,0;y)\\&
+2\,G(0;x,y)\,H(0,0,0;y)\\&
-\left( G(0;x,y)\,H(1,0,0;y) \right) \\&
+\frac{1}{2}\,G(0;x,y)\,H(1,1,0;y)\\&
+\frac{-\left( {\pi }^2\,\left( -1 + x + y \right)  \right) }{24\,\lambda}\,G(\lambda ;0,y)\,G(\lambda ;x,y)\\&
+\frac{{\pi }^2\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{24\,\lambda}\,G(\lambda ;0,y)\,G(x\lambda ;x,y)\\&
+19\,G(\lambda ;0,y)\,H(0;x_0)\\&
-\left( \frac{19}{2} \right) \,G(\lambda ;0,y)\,H(0;y)\\&
+\frac{{\pi }^2}{12}\,G(\lambda ;0,y)\,H(1;y)\\&
-10\,G(\lambda ;0,y)\,H(0,0;x_0)\\&
+5\,G(\lambda ;0,y)\,H(0,0;y)\\&
+\frac{5}{2}\,G(\lambda ;0,y)\,H(1,0;y)\\&
+4\,G(\lambda ;0,y)\,H(0,0,0;x_0)\\&
-2\,G(\lambda ;0,y)\,H(0,0,0;y)\\&
-\left( G(\lambda ;0,y)\,H(1,0,0;y) \right) \\&
+\frac{1}{2}\,G(\lambda ;0,y)\,H(1,1,0;y)\\&
+\frac{{\pi }^2\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{24\,\lambda}\,G(\lambda ;x,y)\,G(x\lambda ;0,y)\\&
+\frac{-5\,\left( -1 + x + y \right) }{2\,\lambda}\,G(\lambda ;x,y)\,G(\lambda ,0;0,y)\\&
+\frac{-1 + x + y}{2\,\lambda}\,G(\lambda ;x,y)\,G(0,\lambda ,0;0,y)\\&
+\frac{-1 + x + y}{2\,\lambda}\,G(\lambda ;x,y)\,G(\lambda ,0,0;0,y)\\&
+\frac{-1 + x + y}{4\,\lambda}\,G(\lambda ;x,y)\,G(\lambda ,0,\lambda ;0,y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{4\,\lambda}\,G(\lambda ;x,y)\,G(\lambda ,0,x\lambda ;0,y)\\&
+\frac{-\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;x,y)\,G(\lambda ,\lambda ,0;0,y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{4\,\lambda}\,G(\lambda ;x,y)\,G(\lambda ,x\lambda ,0;0,y)\\&
+\frac{-1 + x + y}{2\,\lambda}\,G(\lambda ;x,y)\,G(x_0,\lambda ,0;0,y)\\&
+\frac{-1 + x + y}{2\,\lambda}\,G(\lambda ;x,y)\,G(x_1,\lambda ,0;0,y)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{2\,\lambda}\,G(\lambda ;x,y)\,G(x\lambda ,\lambda ,0;0,y)\\&
+\frac{19\,\left( -1 + x + y \right) }{\lambda}\,G(\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-19\,\left( -1 + x + y \right) }{2\,\lambda}\,G(\lambda ;x,y)\,H(0;y)\\&
+\frac{{\pi }^2\,\left( -1 + x + y \right) }{12\,\lambda}\,G(\lambda ;x,y)\,H(1;y)\\&
+\frac{-10\,\left( -1 + x + y \right) }{\lambda}\,G(\lambda ;x,y)\,H(0,0;x_0)\\&
+\frac{5\,\left( -1 + x + y \right) }{\lambda}\,G(\lambda ;x,y)\,H(0,0;y)\\&
+\frac{5\,\left( -1 + x + y \right) }{2\,\lambda}\,G(\lambda ;x,y)\,H(1,0;y)\\&
+\frac{4\,\left( -1 + x + y \right) }{\lambda}\,G(\lambda ;x,y)\,H(0,0,0;x_0)\\&
+\frac{-2\,\left( -1 + x + y \right) }{\lambda}\,G(\lambda ;x,y)\,H(0,0,0;y)\\&
-\left( \frac{-1 + x + y}{\lambda} \right) \,G(\lambda ;x,y)\,H(1,0,0;y)\\&
+\frac{-1 + x + y}{2\,\lambda}\,G(\lambda ;x,y)\,H(1,1,0;y)\\&
+\frac{-\left( {\pi }^2\,{\left( -1 + y \right) }^2\,\left( -1 + x + y \right)  \right) }{24\,\lambda}\,G(x\lambda ;0,y)\,G(x\lambda ;x,y)\\&
+\frac{-19\,\left( -1 + y \right) }{2}\,G(x\lambda ;0,y)\,H(0;y)\\&
+\frac{-\left( {\pi }^2\,\left( -1 + y \right)  \right) }{12}\,G(x\lambda ;0,y)\,H(1;y)\\&
+5\,\left( -1 + y \right) \,G(x\lambda ;0,y)\,H(0,0;y)\\&
+\frac{-5\,\left( -1 + y \right) }{2}\,G(x\lambda ;0,y)\,H(1,0;y)\\&
+(2 - 2\,y)\,G(x\lambda ;0,y)\,H(0,0,0;y)\\&
+(-1 + y)\,G(x\lambda ;0,y)\,H(1,0,0;y)\\&
+\frac{1 - y}{2}\,G(x\lambda ;0,y)\,H(1,1,0;y)\\&
+\frac{5\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{2\,\lambda}\,G(x\lambda ;x,y)\,G(\lambda ,0;0,y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(x\lambda ;x,y)\,G(0,\lambda ,0;0,y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(x\lambda ;x,y)\,G(\lambda ,0,0;0,y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{4\,\lambda}\,G(x\lambda ;x,y)\,G(\lambda ,0,\lambda ;0,y)\\&
+\frac{{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ;x,y)\,G(\lambda ,0,x\lambda ;0,y)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ;x,y)\,G(\lambda ,\lambda ,0;0,y)\\&
+\frac{{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ;x,y)\,G(\lambda ,x\lambda ,0;0,y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(x\lambda ;x,y)\,G(x_0,\lambda ,0;0,y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(x\lambda ;x,y)\,G(x_1,\lambda ,0;0,y)\\&
+\frac{-\left( {\left( -1 + y \right) }^2\,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(x\lambda ;x,y)\,G(x\lambda ,\lambda ,0;0,y)\\&
+\frac{-19\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{2\,\lambda}\,G(x\lambda ;x,y)\,H(0;y)\\&
+\frac{-\left( {\pi }^2\,\left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{12\,\lambda}\,G(x\lambda ;x,y)\,H(1;y)\\&
+\frac{5\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{\lambda}\,G(x\lambda ;x,y)\,H(0,0;y)\\&
+\frac{-5\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{2\,\lambda}\,G(x\lambda ;x,y)\,H(1,0;y)\\&
+\frac{-2\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{\lambda}\,G(x\lambda ;x,y)\,H(0,0,0;y)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{\lambda}\,G(x\lambda ;x,y)\,H(1,0,0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(x\lambda ;x,y)\,H(1,1,0;y)\\&
+\frac{1}{4}\,G(0,0;0,y)\,G(\lambda ,0;0,y)\\&
-\left( \frac{5}{4} \right) \,G(0,0;0,y)\,H(0;y)\\&
+\frac{1}{2}\,G(0,0;0,y)\,H(0,0;y)\\&
-\left( \frac{1}{4} \right) \,G(0,0;0,y)\,H(1,0;y)\\&
+\frac{1}{4}\,G(0,0;x,y)\,G(\lambda ,0;0,y)\\&
-\left( \frac{5}{4} \right) \,G(0,0;x,y)\,H(0;y)\\&
+\frac{1}{2}\,G(0,0;x,y)\,H(0,0;y)\\&
-\left( \frac{1}{4} \right) \,G(0,0;x,y)\,H(1,0;y)\\&
+\frac{1}{4}\,G(0,\lambda ;0,y)\,G(\lambda ,0;0,y)\\&
-5\,G(0,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{15}{4}\,G(0,\lambda ;0,y)\,H(0;y)\\&
+2\,G(0,\lambda ;0,y)\,H(0,0;x_0)\\&
-\left( \frac{3}{2} \right) \,G(0,\lambda ;0,y)\,H(0,0;y)\\&
-\left( \frac{1}{4} \right) \,G(0,\lambda ;0,y)\,H(1,0;y)\\&
+\frac{3\,\left( -1 + x + y \right) }{4\,\lambda}\,G(0,\lambda ;x,y)\,G(\lambda ,0;0,y)\\&
+\frac{-15\,\left( -1 + x + y \right) }{2\,\lambda}\,G(0,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{15\,\left( -1 + x + y \right) }{4\,\lambda}\,G(0,\lambda ;x,y)\,H(0;y)\\&
+\frac{3\,\left( -1 + x + y \right) }{\lambda}\,G(0,\lambda ;x,y)\,H(0,0;x_0)\\&
+\frac{-3\,\left( -1 + x + y \right) }{2\,\lambda}\,G(0,\lambda ;x,y)\,H(0,0;y)\\&
+\frac{-3\,\left( -1 + x + y \right) }{4\,\lambda}\,G(0,\lambda ;x,y)\,H(1,0;y)\\&
+\frac{1 - y}{4}\,G(0,x\lambda ;0,y)\,G(\lambda ,0;0,y)\\&
+\frac{5\,\left( -1 + y \right) }{4}\,G(0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{1 - y}{2}\,G(0,x\lambda ;0,y)\,H(0,0;y)\\&
+\frac{-1 + y}{4}\,G(0,x\lambda ;0,y)\,H(1,0;y)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(0,x\lambda ;x,y)\,G(\lambda ,0;0,y)\\&
+\frac{15\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(0,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{2\,\lambda}\,G(0,x\lambda ;x,y)\,H(0,0;y)\\&
+\frac{3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(0,x\lambda ;x,y)\,H(1,0;y)\\&
-\left( \frac{1}{4} \right) \,{G(\lambda ,0;0,y)}^2\\&
+\frac{-1 + x + y}{4\,\lambda}\,G(\lambda ,0;0,y)\,G(\lambda ,0;x,y)\\&
-\left( \frac{1}{4} \right) \,G(\lambda ,0;0,y)\,G(\lambda ,\lambda ;0,y)\\&
+\frac{3}{4}\,G(\lambda ,0;0,y)\,G(\lambda ,\lambda ;x,y)\\&
+\frac{-1 + y}{4}\,G(\lambda ,0;0,y)\,G(\lambda ,x\lambda ;0,y)\\&
+\frac{-3\,\left( -1 + y \right) }{4}\,G(\lambda ,0;0,y)\,G(\lambda ,x\lambda ;x,y)\\&
+\frac{1}{2}\,G(\lambda ,0;0,y)\,G(x_0,\lambda ;0,y)\\&
+\frac{-1 + x + y}{2\,\lambda}\,G(\lambda ,0;0,y)\,G(x_0,\lambda ;x,y)\\&
+\frac{1 - y}{2}\,G(\lambda ,0;0,y)\,G(x_0,x\lambda ;0,y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(\lambda ,0;0,y)\,G(x_0,x\lambda ;x,y)\\&
+\frac{1}{2}\,G(\lambda ,0;0,y)\,G(x_1,\lambda ;0,y)\\&
+\frac{-1 + x + y}{2\,\lambda}\,G(\lambda ,0;0,y)\,G(x_1,\lambda ;x,y)\\&
+\frac{1 - y}{2}\,G(\lambda ,0;0,y)\,G(x_1,x\lambda ;0,y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(\lambda ,0;0,y)\,G(x_1,x\lambda ;x,y)\\&
+\frac{-1 + y}{4}\,G(\lambda ,0;0,y)\,G(x\lambda ,0;0,y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{4\,\lambda}\,G(\lambda ,0;0,y)\,G(x\lambda ,0;x,y)\\&
+\frac{-1 + y}{4}\,G(\lambda ,0;0,y)\,G(x\lambda ,\lambda ;0,y)\\&
+\frac{-3\,\left( -1 + y \right) }{4}\,G(\lambda ,0;0,y)\,G(x\lambda ,\lambda ;x,y)\\&
+\frac{-{\left( -1 + y \right) }^2}{4}\,G(\lambda ,0;0,y)\,G(x\lambda ,x\lambda ;0,y)\\&
+\frac{3\,{\left( -1 + y \right) }^2}{4}\,G(\lambda ,0;0,y)\,G(x\lambda ,x\lambda ;x,y)\\&
-\left( \frac{15}{2} \right) \,G(\lambda ,0;0,y)\,H(0;x_0)\\&
-\left( \frac{5}{4} \right) \,G(\lambda ,0;0,y)\,H(0;y)\\&
+3\,G(\lambda ,0;0,y)\,H(0,0;x_0)\\&
+\frac{1}{2}\,G(\lambda ,0;0,y)\,H(0,0;y)\\&
+\frac{1}{4}\,G(\lambda ,0;0,y)\,H(1,0;y)\\&
+\frac{-10\,\left( -1 + x + y \right) }{\lambda}\,G(\lambda ,0;x,y)\,H(0;x_0)\\&
+\frac{-5\,\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ,0;x,y)\,H(0;y)\\&
+\frac{4\,\left( -1 + x + y \right) }{\lambda}\,G(\lambda ,0;x,y)\,H(0,0;x_0)\\&
+\frac{-1 + x + y}{2\,\lambda}\,G(\lambda ,0;x,y)\,H(0,0;y)\\&
+\frac{-\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ,0;x,y)\,H(1,0;y)\\&
+\frac{5}{2}\,G(\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
-\left( \frac{5}{4} \right) \,G(\lambda ,\lambda ;0,y)\,H(0;y)\\&
-\left( G(\lambda ,\lambda ;0,y)\,H(0,0;x_0) \right) \\&
+\frac{1}{2}\,G(\lambda ,\lambda ;0,y)\,H(0,0;y)\\&
+\frac{1}{4}\,G(\lambda ,\lambda ;0,y)\,H(1,0;y)\\&
-\left( \frac{15}{2} \right) \,G(\lambda ,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{15}{4}\,G(\lambda ,\lambda ;x,y)\,H(0;y)\\&
+3\,G(\lambda ,\lambda ;x,y)\,H(0,0;x_0)\\&
-\left( \frac{3}{2} \right) \,G(\lambda ,\lambda ;x,y)\,H(0,0;y)\\&
-\left( \frac{3}{4} \right) \,G(\lambda ,\lambda ;x,y)\,H(1,0;y)\\&
+\frac{5\,\left( -1 + y \right) }{2}\,G(\lambda ,x\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-15\,\left( -1 + y \right) }{4}\,G(\lambda ,x\lambda ;0,y)\,H(0;y)\\&
+(1 - y)\,G(\lambda ,x\lambda ;0,y)\,H(0,0;x_0)\\&
+\frac{3\,\left( -1 + y \right) }{2}\,G(\lambda ,x\lambda ;0,y)\,H(0,0;y)\\&
+\frac{1 - y}{4}\,G(\lambda ,x\lambda ;0,y)\,H(1,0;y)\\&
+\frac{15\,\left( -1 + y \right) }{4}\,G(\lambda ,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) }{2}\,G(\lambda ,x\lambda ;x,y)\,H(0,0;y)\\&
+\frac{3\,\left( -1 + y \right) }{4}\,G(\lambda ,x\lambda ;x,y)\,H(1,0;y)\\&
-5\,G(x_0,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{5}{2}\,G(x_0,\lambda ;0,y)\,H(0;y)\\&
+2\,G(x_0,\lambda ;0,y)\,H(0,0;x_0)\\&
-\left( G(x_0,\lambda ;0,y)\,H(0,0;y) \right) \\&
-\left( \frac{1}{2} \right) \,G(x_0,\lambda ;0,y)\,H(1,0;y)\\&
+\frac{-5\,\left( -1 + x + y \right) }{\lambda}\,G(x_0,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{5\,\left( -1 + x + y \right) }{2\,\lambda}\,G(x_0,\lambda ;x,y)\,H(0;y)\\&
+\frac{2\,\left( -1 + x + y \right) }{\lambda}\,G(x_0,\lambda ;x,y)\,H(0,0;x_0)\\&
-\left( \frac{-1 + x + y}{\lambda} \right) \,G(x_0,\lambda ;x,y)\,H(0,0;y)\\&
+\frac{-\left( -1 + x + y \right) }{2\,\lambda}\,G(x_0,\lambda ;x,y)\,H(1,0;y)\\&
+\frac{5\,\left( -1 + y \right) }{2}\,G(x_0,x\lambda ;0,y)\,H(0;y)\\&
+(1 - y)\,G(x_0,x\lambda ;0,y)\,H(0,0;y)\\&
+\frac{-1 + y}{2}\,G(x_0,x\lambda ;0,y)\,H(1,0;y)\\&
+\frac{5\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{2\,\lambda}\,G(x_0,x\lambda ;x,y)\,H(0;y)\\&
-\left( \frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{\lambda} \right) \,G(x_0,x\lambda ;x,y)\,H(0,0;y)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{2\,\lambda}\,G(x_0,x\lambda ;x,y)\,H(1,0;y)\\&
-5\,G(x_1,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{5}{2}\,G(x_1,\lambda ;0,y)\,H(0;y)\\&
+2\,G(x_1,\lambda ;0,y)\,H(0,0;x_0)\\&
-\left( G(x_1,\lambda ;0,y)\,H(0,0;y) \right) \\&
-\left( \frac{1}{2} \right) \,G(x_1,\lambda ;0,y)\,H(1,0;y)\\&
+\frac{-5\,\left( -1 + x + y \right) }{\lambda}\,G(x_1,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{5\,\left( -1 + x + y \right) }{2\,\lambda}\,G(x_1,\lambda ;x,y)\,H(0;y)\\&
+\frac{2\,\left( -1 + x + y \right) }{\lambda}\,G(x_1,\lambda ;x,y)\,H(0,0;x_0)\\&
-\left( \frac{-1 + x + y}{\lambda} \right) \,G(x_1,\lambda ;x,y)\,H(0,0;y)\\&
+\frac{-\left( -1 + x + y \right) }{2\,\lambda}\,G(x_1,\lambda ;x,y)\,H(1,0;y)\\&
+\frac{5\,\left( -1 + y \right) }{2}\,G(x_1,x\lambda ;0,y)\,H(0;y)\\&
+(1 - y)\,G(x_1,x\lambda ;0,y)\,H(0,0;y)\\&
+\frac{-1 + y}{2}\,G(x_1,x\lambda ;0,y)\,H(1,0;y)\\&
+\frac{5\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{2\,\lambda}\,G(x_1,x\lambda ;x,y)\,H(0;y)\\&
-\left( \frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{\lambda} \right) \,G(x_1,x\lambda ;x,y)\,H(0,0;y)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{2\,\lambda}\,G(x_1,x\lambda ;x,y)\,H(1,0;y)\\&
+\frac{-5\,\left( -1 + y \right) }{4}\,G(x\lambda ,0;0,y)\,H(0;y)\\&
+\frac{-1 + y}{2}\,G(x\lambda ,0;0,y)\,H(0,0;y)\\&
+\frac{1 - y}{4}\,G(x\lambda ,0;0,y)\,H(1,0;y)\\&
+\frac{5\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ,0;x,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(x\lambda ,0;x,y)\,H(0,0;y)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ,0;x,y)\,H(1,0;y)\\&
+(5 - 5\,y)\,G(x\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{15\,\left( -1 + y \right) }{4}\,G(x\lambda ,\lambda ;0,y)\,H(0;y)\\&
+2\,\left( -1 + y \right) \,G(x\lambda ,\lambda ;0,y)\,H(0,0;x_0)\\&
+\frac{-3\,\left( -1 + y \right) }{2}\,G(x\lambda ,\lambda ;0,y)\,H(0,0;y)\\&
+\frac{1 - y}{4}\,G(x\lambda ,\lambda ;0,y)\,H(1,0;y)\\&
+\frac{15\,\left( -1 + y \right) }{2}\,G(x\lambda ,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-15\,\left( -1 + y \right) }{4}\,G(x\lambda ,\lambda ;x,y)\,H(0;y)\\&
+(3 - 3\,y)\,G(x\lambda ,\lambda ;x,y)\,H(0,0;x_0)\\&
+\frac{3\,\left( -1 + y \right) }{2}\,G(x\lambda ,\lambda ;x,y)\,H(0,0;y)\\&
+\frac{3\,\left( -1 + y \right) }{4}\,G(x\lambda ,\lambda ;x,y)\,H(1,0;y)\\&
+\frac{5\,{\left( -1 + y \right) }^2}{4}\,G(x\lambda ,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-{\left( -1 + y \right) }^2}{2}\,G(x\lambda ,x\lambda ;0,y)\,H(0,0;y)\\&
+\frac{{\left( -1 + y \right) }^2}{4}\,G(x\lambda ,x\lambda ;0,y)\,H(1,0;y)\\&
+\frac{-15\,{\left( -1 + y \right) }^2}{4}\,G(x\lambda ,x\lambda ;x,y)\,H(0;y)\\&
+\frac{3\,{\left( -1 + y \right) }^2}{2}\,G(x\lambda ,x\lambda ;x,y)\,H(0,0;y)\\&
+\frac{-3\,{\left( -1 + y \right) }^2}{4}\,G(x\lambda ,x\lambda ;x,y)\,H(1,0;y)\\&
-\left( \frac{1}{8} \right) \,G(0,0,0;0,y)\,H(0;y)\\&
+\frac{1}{8}\,G(0,0,0;x,y)\,H(0;y)\\&
+G(0,0,\lambda ;0,y)\,H(0;x_0)\\&
-\left( \frac{7}{8} \right) \,G(0,0,\lambda ;0,y)\,H(0;y)\\&
+\frac{9\,\left( -1 + x + y \right) }{4\,\lambda}\,G(0,0,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-9\,\left( -1 + x + y \right) }{8\,\lambda}\,G(0,0,\lambda ;x,y)\,H(0;y)\\&
+\frac{1 - y}{8}\,G(0,0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-9\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{8\,\lambda}\,G(0,0,x\lambda ;x,y)\,H(0;y)\\&
+\frac{3}{2}\,G(0,\lambda ,0;0,y)\,H(0;x_0)\\&
+\frac{3}{8}\,G(0,\lambda ,0;0,y)\,H(0;y)\\&
+\frac{3\,\left( -1 + x + y \right) }{\lambda}\,G(0,\lambda ,0;x,y)\,H(0;x_0)\\&
+\frac{3\,\left( -1 + x + y \right) }{8\,\lambda}\,G(0,\lambda ,0;x,y)\,H(0;y)\\&
+2\,G(0,\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
-\left( \frac{7}{8} \right) \,G(0,\lambda ,\lambda ;0,y)\,H(0;y)\\&
+\frac{3}{4}\,G(0,\lambda ,\lambda ;x,y)\,H(0;x_0)\\&
-\left( \frac{3}{8} \right) \,G(0,\lambda ,\lambda ;x,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) }{2}\,G(0,\lambda ,x\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-3\,\left( -1 + y \right) }{8}\,G(0,\lambda ,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) }{8}\,G(0,\lambda ,x\lambda ;x,y)\,H(0;y)\\&
+G(0,x_0,\lambda ;0,y)\,H(0;x_0)\\&
-\left( \frac{3}{4} \right) \,G(0,x_0,\lambda ;0,y)\,H(0;y)\\&
+\frac{3\,\left( -1 + x + y \right) }{2\,\lambda}\,G(0,x_0,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-3\,\left( -1 + x + y \right) }{4\,\lambda}\,G(0,x_0,\lambda ;x,y)\,H(0;y)\\&
+\frac{1 - y}{4}\,G(0,x_0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(0,x_0,x\lambda ;x,y)\,H(0;y)\\&
+G(0,x_1,\lambda ;0,y)\,H(0;x_0)\\&
-\left( \frac{3}{4} \right) \,G(0,x_1,\lambda ;0,y)\,H(0;y)\\&
+\frac{3\,\left( -1 + x + y \right) }{2\,\lambda}\,G(0,x_1,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-3\,\left( -1 + x + y \right) }{4\,\lambda}\,G(0,x_1,\lambda ;x,y)\,H(0;y)\\&
+\frac{1 - y}{4}\,G(0,x_1,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(0,x_1,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-1 + y}{8}\,G(0,x\lambda ,0;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{8\,\lambda}\,G(0,x\lambda ,0;x,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) }{2}\,G(0,x\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-3\,\left( -1 + y \right) }{8}\,G(0,x\lambda ,\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) }{4}\,G(0,x\lambda ,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{3\,\left( -1 + y \right) }{8}\,G(0,x\lambda ,\lambda ;x,y)\,H(0;y)\\&
+\frac{9\,{\left( -1 + y \right) }^2}{8}\,G(0,x\lambda ,x\lambda ;0,y)\,H(0;y)\\&
+\frac{3\,{\left( -1 + y \right) }^2}{8}\,G(0,x\lambda ,x\lambda ;x,y)\,H(0;y)\\&
+\frac{9}{4}\,G(\lambda ,0,0;0,y)\,H(0;x_0)\\&
-\left( \frac{1}{8} \right) \,G(\lambda ,0,0;0,y)\,H(0;y)\\&
+\frac{4\,\left( -1 + x + y \right) }{\lambda}\,G(\lambda ,0,0;x,y)\,H(0;x_0)\\&
+\frac{-1 + x + y}{8\,\lambda}\,G(\lambda ,0,0;x,y)\,H(0;y)\\&
+\frac{1}{4}\,G(\lambda ,0,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{5}{8}\,G(\lambda ,0,\lambda ;0,y)\,H(0;y)\\&
+\frac{9}{4}\,G(\lambda ,0,\lambda ;x,y)\,H(0;x_0)\\&
-\left( \frac{9}{8} \right) \,G(\lambda ,0,\lambda ;x,y)\,H(0;y)\\&
+\frac{-7\,\left( -1 + y \right) }{4}\,G(\lambda ,0,x\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-1 + y}{8}\,G(\lambda ,0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-9\,\left( -1 + y \right) }{8}\,G(\lambda ,0,x\lambda ;x,y)\,H(0;y)\\&
-\left( \frac{3}{4} \right) \,G(\lambda ,\lambda ,0;0,y)\,H(0;x_0)\\&
-\left( \frac{1}{8} \right) \,G(\lambda ,\lambda ,0;0,y)\,H(0;y)\\&
+3\,G(\lambda ,\lambda ,0;x,y)\,H(0;x_0)\\&
+\frac{3}{8}\,G(\lambda ,\lambda ,0;x,y)\,H(0;y)\\&
-\left( \frac{9}{4} \right) \,G(\lambda ,\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{9}{8}\,G(\lambda ,\lambda ,\lambda ;0,y)\,H(0;y)\\&
+\frac{3\,\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ,\lambda ,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-3\,\left( -1 + x + y \right) }{8\,\lambda}\,G(\lambda ,\lambda ,\lambda ;x,y)\,H(0;y)\\&
+\frac{5\,\left( -1 + y \right) }{4}\,G(\lambda ,\lambda ,x\lambda ;0,y)\,H(0;x_0)\\&
+\frac{1 - y}{8}\,G(\lambda ,\lambda ,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{8\,\lambda}\,G(\lambda ,\lambda ,x\lambda ;x,y)\,H(0;y)\\&
-\left( \frac{1}{2} \right) \,G(\lambda ,x_0,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{1}{4}\,G(\lambda ,x_0,\lambda ;0,y)\,H(0;y)\\&
+\frac{3}{2}\,G(\lambda ,x_0,\lambda ;x,y)\,H(0;x_0)\\&
-\left( \frac{3}{4} \right) \,G(\lambda ,x_0,\lambda ;x,y)\,H(0;y)\\&
+\frac{1 - y}{2}\,G(\lambda ,x_0,x\lambda ;0,y)\,H(0;x_0)\\&
+\frac{3\,\left( -1 + y \right) }{4}\,G(\lambda ,x_0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) }{4}\,G(\lambda ,x_0,x\lambda ;x,y)\,H(0;y)\\&
-\left( \frac{1}{2} \right) \,G(\lambda ,x_1,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{1}{4}\,G(\lambda ,x_1,\lambda ;0,y)\,H(0;y)\\&
+\frac{3}{2}\,G(\lambda ,x_1,\lambda ;x,y)\,H(0;x_0)\\&
-\left( \frac{3}{4} \right) \,G(\lambda ,x_1,\lambda ;x,y)\,H(0;y)\\&
+\frac{1 - y}{2}\,G(\lambda ,x_1,x\lambda ;0,y)\,H(0;x_0)\\&
+\frac{3\,\left( -1 + y \right) }{4}\,G(\lambda ,x_1,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) }{4}\,G(\lambda ,x_1,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-5\,\left( -1 + y \right) }{4}\,G(\lambda ,x\lambda ,0;0,y)\,H(0;x_0)\\&
+\frac{-5\,\left( -1 + y \right) }{8}\,G(\lambda ,x\lambda ,0;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) }{8}\,G(\lambda ,x\lambda ,0;x,y)\,H(0;y)\\&
+\frac{5\,\left( -1 + y \right) }{4}\,G(\lambda ,x\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{1 - y}{8}\,G(\lambda ,x\lambda ,\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ,x\lambda ,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{8\,\lambda}\,G(\lambda ,x\lambda ,\lambda ;x,y)\,H(0;y)\\&
+\frac{-{\left( -1 + y \right) }^2}{4}\,G(\lambda ,x\lambda ,x\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-7\,{\left( -1 + y \right) }^2}{8}\,G(\lambda ,x\lambda ,x\lambda ;0,y)\,H(0;y)\\&
+\frac{3\,{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{8\,\lambda}\,G(\lambda ,x\lambda ,x\lambda ;x,y)\,H(0;y)\\&
+G(x_0,0,\lambda ;0,y)\,H(0;x_0)\\&
-\left( \frac{3}{4} \right) \,G(x_0,0,\lambda ;0,y)\,H(0;y)\\&
+\frac{3\,\left( -1 + x + y \right) }{2\,\lambda}\,G(x_0,0,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-3\,\left( -1 + x + y \right) }{4\,\lambda}\,G(x_0,0,\lambda ;x,y)\,H(0;y)\\&
+\frac{1 - y}{4}\,G(x_0,0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(x_0,0,x\lambda ;x,y)\,H(0;y)\\&
+\frac{3}{2}\,G(x_0,\lambda ,0;0,y)\,H(0;x_0)\\&
+\frac{1}{4}\,G(x_0,\lambda ,0;0,y)\,H(0;y)\\&
+\frac{2\,\left( -1 + x + y \right) }{\lambda}\,G(x_0,\lambda ,0;x,y)\,H(0;x_0)\\&
+\frac{-1 + x + y}{4\,\lambda}\,G(x_0,\lambda ,0;x,y)\,H(0;y)\\&
+2\,G(x_0,\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
-\left( G(x_0,\lambda ,\lambda ;0,y)\,H(0;y) \right) \\&
+(1 - y)\,G(x_0,\lambda ,x\lambda ;0,y)\,H(0;x_0)\\&
+G(x_0,x_0,\lambda ;0,y)\,H(0;x_0)\\&
-\left( \frac{1}{2} \right) \,G(x_0,x_0,\lambda ;0,y)\,H(0;y)\\&
+\frac{-1 + x + y}{\lambda}\,G(x_0,x_0,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-\left( -1 + x + y \right) }{2\,\lambda}\,G(x_0,x_0,\lambda ;x,y)\,H(0;y)\\&
+\frac{1 - y}{2}\,G(x_0,x_0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(x_0,x_0,x\lambda ;x,y)\,H(0;y)\\&
+G(x_0,x_1,\lambda ;0,y)\,H(0;x_0)\\&
-\left( \frac{1}{2} \right) \,G(x_0,x_1,\lambda ;0,y)\,H(0;y)\\&
+\frac{-1 + x + y}{\lambda}\,G(x_0,x_1,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-\left( -1 + x + y \right) }{2\,\lambda}\,G(x_0,x_1,\lambda ;x,y)\,H(0;y)\\&
+\frac{1 - y}{2}\,G(x_0,x_1,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(x_0,x_1,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-1 + y}{4}\,G(x_0,x\lambda ,0;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{4\,\lambda}\,G(x_0,x\lambda ,0;x,y)\,H(0;y)\\&
+(1 - y)\,G(x_0,x\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
+{\left( -1 + y \right) }^2\,G(x_0,x\lambda ,x\lambda ;0,y)\,H(0;y)\\&
+G(x_1,0,\lambda ;0,y)\,H(0;x_0)\\&
-\left( \frac{3}{4} \right) \,G(x_1,0,\lambda ;0,y)\,H(0;y)\\&
+\frac{3\,\left( -1 + x + y \right) }{2\,\lambda}\,G(x_1,0,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-3\,\left( -1 + x + y \right) }{4\,\lambda}\,G(x_1,0,\lambda ;x,y)\,H(0;y)\\&
+\frac{1 - y}{4}\,G(x_1,0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(x_1,0,x\lambda ;x,y)\,H(0;y)\\&
+\frac{3}{2}\,G(x_1,\lambda ,0;0,y)\,H(0;x_0)\\&
+\frac{1}{4}\,G(x_1,\lambda ,0;0,y)\,H(0;y)\\&
+\frac{2\,\left( -1 + x + y \right) }{\lambda}\,G(x_1,\lambda ,0;x,y)\,H(0;x_0)\\&
+\frac{-1 + x + y}{4\,\lambda}\,G(x_1,\lambda ,0;x,y)\,H(0;y)\\&
+2\,G(x_1,\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
-\left( G(x_1,\lambda ,\lambda ;0,y)\,H(0;y) \right) \\&
+(1 - y)\,G(x_1,\lambda ,x\lambda ;0,y)\,H(0;x_0)\\&
+G(x_1,x_0,\lambda ;0,y)\,H(0;x_0)\\&
-\left( \frac{1}{2} \right) \,G(x_1,x_0,\lambda ;0,y)\,H(0;y)\\&
+\frac{-1 + x + y}{\lambda}\,G(x_1,x_0,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-\left( -1 + x + y \right) }{2\,\lambda}\,G(x_1,x_0,\lambda ;x,y)\,H(0;y)\\&
+\frac{1 - y}{2}\,G(x_1,x_0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(x_1,x_0,x\lambda ;x,y)\,H(0;y)\\&
+G(x_1,x_1,\lambda ;0,y)\,H(0;x_0)\\&
-\left( \frac{1}{2} \right) \,G(x_1,x_1,\lambda ;0,y)\,H(0;y)\\&
+\frac{-1 + x + y}{\lambda}\,G(x_1,x_1,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-\left( -1 + x + y \right) }{2\,\lambda}\,G(x_1,x_1,\lambda ;x,y)\,H(0;y)\\&
+\frac{1 - y}{2}\,G(x_1,x_1,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(x_1,x_1,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-1 + y}{4}\,G(x_1,x\lambda ,0;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{4\,\lambda}\,G(x_1,x\lambda ,0;x,y)\,H(0;y)\\&
+(1 - y)\,G(x_1,x\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
+{\left( -1 + y \right) }^2\,G(x_1,x\lambda ,x\lambda ;0,y)\,H(0;y)\\&
+\frac{1 - y}{8}\,G(x\lambda ,0,0;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{8\,\lambda}\,G(x\lambda ,0,0;x,y)\,H(0;y)\\&
+\frac{-1 + y}{2}\,G(x\lambda ,0,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-9\,\left( -1 + y \right) }{8}\,G(x\lambda ,0,\lambda ;0,y)\,H(0;y)\\&
+\frac{-9\,\left( -1 + y \right) }{4}\,G(x\lambda ,0,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{9\,\left( -1 + y \right) }{8}\,G(x\lambda ,0,\lambda ;x,y)\,H(0;y)\\&
+\frac{-{\left( -1 + y \right) }^2}{8}\,G(x\lambda ,0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{9\,{\left( -1 + y \right) }^2}{8}\,G(x\lambda ,0,x\lambda ;x,y)\,H(0;y)\\&
+(-1 + y)\,G(x\lambda ,\lambda ,0;0,y)\,H(0;x_0)\\&
+\frac{-1 + y}{8}\,G(x\lambda ,\lambda ,0;0,y)\,H(0;y)\\&
+(3 - 3\,y)\,G(x\lambda ,\lambda ,0;x,y)\,H(0;x_0)\\&
+\frac{-3\,\left( -1 + y \right) }{8}\,G(x\lambda ,\lambda ,0;x,y)\,H(0;y)\\&
+2\,\left( -1 + y \right) \,G(x\lambda ,\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-7\,\left( -1 + y \right) }{8}\,G(x\lambda ,\lambda ,\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ,\lambda ,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{8\,\lambda}\,G(x\lambda ,\lambda ,\lambda ;x,y)\,H(0;y)\\&
-{\left( -1 + y \right) }^2\,G(x\lambda ,\lambda ,x\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-{\left( -1 + y \right) }^2}{8}\,G(x\lambda ,\lambda ,x\lambda ;0,y)\,H(0;y)\\&
+\frac{3\,{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{8\,\lambda}\,G(x\lambda ,\lambda ,x\lambda ;x,y)\,H(0;y)\\&
+(-1 + y)\,G(x\lambda ,x_0,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-3\,\left( -1 + y \right) }{4}\,G(x\lambda ,x_0,\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) }{2}\,G(x\lambda ,x_0,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{3\,\left( -1 + y \right) }{4}\,G(x\lambda ,x_0,\lambda ;x,y)\,H(0;y)\\&
+\frac{-{\left( -1 + y \right) }^2}{4}\,G(x\lambda ,x_0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{3\,{\left( -1 + y \right) }^2}{4}\,G(x\lambda ,x_0,x\lambda ;x,y)\,H(0;y)\\&
+(-1 + y)\,G(x\lambda ,x_1,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-3\,\left( -1 + y \right) }{4}\,G(x\lambda ,x_1,\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) }{2}\,G(x\lambda ,x_1,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{3\,\left( -1 + y \right) }{4}\,G(x\lambda ,x_1,\lambda ;x,y)\,H(0;y)\\&
+\frac{-{\left( -1 + y \right) }^2}{4}\,G(x\lambda ,x_1,x\lambda ;0,y)\,H(0;y)\\&
+\frac{3\,{\left( -1 + y \right) }^2}{4}\,G(x\lambda ,x_1,x\lambda ;x,y)\,H(0;y)\\&
+\frac{{\left( -1 + y \right) }^2}{8}\,G(x\lambda ,x\lambda ,0;0,y)\,H(0;y)\\&
+\frac{3\,{\left( -1 + y \right) }^2}{8}\,G(x\lambda ,x\lambda ,0;x,y)\,H(0;y)\\&
-{\left( -1 + y \right) }^2\,G(x\lambda ,x\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-{\left( -1 + y \right) }^2}{8}\,G(x\lambda ,x\lambda ,\lambda ;0,y)\,H(0;y)\\&
+\frac{3\,{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ,x\lambda ,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-3\,{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{8\,\lambda}\,G(x\lambda ,x\lambda ,\lambda ;x,y)\,H(0;y)\\&
+\frac{9\,{\left( -1 + y \right) }^3}{8}\,G(x\lambda ,x\lambda ,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,{\left( -1 + y \right) }^3\,\left( -1 + x + y \right) }{8\,\lambda}\,G(x\lambda ,x\lambda ,x\lambda ;x,y)\,H(0;y)\\&
+\frac{5}{4}\,G(0;0,y)\,G(0;x,y)\,H(0;y)\\&
-\left( \frac{1}{2} \right) \,G(0;0,y)\,G(0;x,y)\,H(0,0;y)\\&
+\frac{1}{4}\,G(0;0,y)\,G(0;x,y)\,H(1,0;y)\\&
+\frac{5\,\left( -1 + x + y \right) }{4\,\lambda}\,G(0;0,y)\,G(\lambda ;x,y)\,H(0;y)\\&
+\frac{-\left( -1 + x + y \right) }{2\,\lambda}\,G(0;0,y)\,G(\lambda ;x,y)\,H(0,0;y)\\&
+\frac{-1 + x + y}{4\,\lambda}\,G(0;0,y)\,G(\lambda ;x,y)\,H(1,0;y)\\&
+\frac{-5\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(0;0,y)\,G(x\lambda ;x,y)\,H(0;y)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{2\,\lambda}\,G(0;0,y)\,G(x\lambda ;x,y)\,H(0,0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{4\,\lambda}\,G(0;0,y)\,G(x\lambda ;x,y)\,H(1,0;y)\\&
-\left( \frac{1}{8} \right) \,G(0;0,y)\,G(0,0;x,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + x + y \right) }{8\,\lambda}\,G(0;0,y)\,G(0,\lambda ;x,y)\,H(0;y)\\&
+\frac{3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{8\,\lambda}\,G(0;0,y)\,G(0,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-\left( -1 + x + y \right) }{8\,\lambda}\,G(0;0,y)\,G(\lambda ,0;x,y)\,H(0;y)\\&
-\left( \frac{3}{8} \right) \,G(0;0,y)\,G(\lambda ,\lambda ;x,y)\,H(0;y)\\&
+\frac{3\,\left( -1 + y \right) }{8}\,G(0;0,y)\,G(\lambda ,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-\left( -1 + x + y \right) }{4\,\lambda}\,G(0;0,y)\,G(x_0,\lambda ;x,y)\,H(0;y)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(0;0,y)\,G(x_0,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-\left( -1 + x + y \right) }{4\,\lambda}\,G(0;0,y)\,G(x_1,\lambda ;x,y)\,H(0;y)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(0;0,y)\,G(x_1,x\lambda ;x,y)\,H(0;y)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{8\,\lambda}\,G(0;0,y)\,G(x\lambda ,0;x,y)\,H(0;y)\\&
+\frac{3\,\left( -1 + y \right) }{8}\,G(0;0,y)\,G(x\lambda ,\lambda ;x,y)\,H(0;y)\\&
+\frac{-3\,{\left( -1 + y \right) }^2}{8}\,G(0;0,y)\,G(x\lambda ,x\lambda ;x,y)\,H(0;y)\\&
-\left( \frac{5}{2} \right) \,G(0;x,y)\,G(\lambda ;0,y)\,H(0;x_0)\\&
+\frac{5}{4}\,G(0;x,y)\,G(\lambda ;0,y)\,H(0;y)\\&
+G(0;x,y)\,G(\lambda ;0,y)\,H(0,0;x_0)\\&
-\left( \frac{1}{2} \right) \,G(0;x,y)\,G(\lambda ;0,y)\,H(0,0;y)\\&
-\left( \frac{1}{4} \right) \,G(0;x,y)\,G(\lambda ;0,y)\,H(1,0;y)\\&
+\frac{5\,\left( -1 + y \right) }{4}\,G(0;x,y)\,G(x\lambda ;0,y)\,H(0;y)\\&
+\frac{1 - y}{2}\,G(0;x,y)\,G(x\lambda ;0,y)\,H(0,0;y)\\&
+\frac{-1 + y}{4}\,G(0;x,y)\,G(x\lambda ;0,y)\,H(1,0;y)\\&
+\frac{1}{8}\,G(0;x,y)\,G(0,0;0,y)\,H(0;y)\\&
+\frac{1}{2}\,G(0;x,y)\,G(0,\lambda ;0,y)\,H(0;x_0)\\&
-\left( \frac{3}{8} \right) \,G(0;x,y)\,G(0,\lambda ;0,y)\,H(0;y)\\&
+\frac{1 - y}{8}\,G(0;x,y)\,G(0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{3}{4}\,G(0;x,y)\,G(\lambda ,0;0,y)\,H(0;x_0)\\&
+\frac{1}{8}\,G(0;x,y)\,G(\lambda ,0;0,y)\,H(0;y)\\&
-\left( \frac{1}{4} \right) \,G(0;x,y)\,G(\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{1}{8}\,G(0;x,y)\,G(\lambda ,\lambda ;0,y)\,H(0;y)\\&
+\frac{1 - y}{4}\,G(0;x,y)\,G(\lambda ,x\lambda ;0,y)\,H(0;x_0)\\&
+\frac{3\,\left( -1 + y \right) }{8}\,G(0;x,y)\,G(\lambda ,x\lambda ;0,y)\,H(0;y)\\&
+\frac{1}{2}\,G(0;x,y)\,G(x_0,\lambda ;0,y)\,H(0;x_0)\\&
-\left( \frac{1}{4} \right) \,G(0;x,y)\,G(x_0,\lambda ;0,y)\,H(0;y)\\&
+\frac{1 - y}{4}\,G(0;x,y)\,G(x_0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{1}{2}\,G(0;x,y)\,G(x_1,\lambda ;0,y)\,H(0;x_0)\\&
-\left( \frac{1}{4} \right) \,G(0;x,y)\,G(x_1,\lambda ;0,y)\,H(0;y)\\&
+\frac{1 - y}{4}\,G(0;x,y)\,G(x_1,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-1 + y}{8}\,G(0;x,y)\,G(x\lambda ,0;0,y)\,H(0;y)\\&
+\frac{-1 + y}{2}\,G(0;x,y)\,G(x\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-3\,\left( -1 + y \right) }{8}\,G(0;x,y)\,G(x\lambda ,\lambda ;0,y)\,H(0;y)\\&
+\frac{-{\left( -1 + y \right) }^2}{8}\,G(0;x,y)\,G(x\lambda ,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-5\,\left( -1 + x + y \right) }{2\,\lambda}\,G(\lambda ;0,y)\,G(\lambda ;x,y)\,H(0;x_0)\\&
+\frac{5\,\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;0,y)\,G(\lambda ;x,y)\,H(0;y)\\&
+\frac{-1 + x + y}{\lambda}\,G(\lambda ;0,y)\,G(\lambda ;x,y)\,H(0,0;x_0)\\&
+\frac{-\left( -1 + x + y \right) }{2\,\lambda}\,G(\lambda ;0,y)\,G(\lambda ;x,y)\,H(0,0;y)\\&
+\frac{-\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;0,y)\,G(\lambda ;x,y)\,H(1,0;y)\\&
+\frac{5\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{2\,\lambda}\,G(\lambda ;0,y)\,G(x\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-5\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;0,y)\,G(x\lambda ;x,y)\,H(0;y)\\&
-\left( \frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{\lambda} \right) \,G(\lambda ;0,y)\,G(x\lambda ;x,y)\,H(0,0;x_0)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{2\,\lambda}\,G(\lambda ;0,y)\,G(x\lambda ;x,y)\,H(0,0;y)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;0,y)\,G(x\lambda ;x,y)\,H(1,0;y)\\&
+\frac{1}{4}\,G(\lambda ;0,y)\,G(0,0;x,y)\,H(0;x_0)\\&
-\left( \frac{1}{8} \right) \,G(\lambda ;0,y)\,G(0,0;x,y)\,H(0;y)\\&
+\frac{3\,\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;0,y)\,G(0,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-3\,\left( -1 + x + y \right) }{8\,\lambda}\,G(\lambda ;0,y)\,G(0,\lambda ;x,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;0,y)\,G(0,x\lambda ;x,y)\,H(0;x_0)\\&
+\frac{3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{8\,\lambda}\,G(\lambda ;0,y)\,G(0,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-1 + x + y}{4\,\lambda}\,G(\lambda ;0,y)\,G(\lambda ,0;x,y)\,H(0;x_0)\\&
+\frac{-\left( -1 + x + y \right) }{8\,\lambda}\,G(\lambda ;0,y)\,G(\lambda ,0;x,y)\,H(0;y)\\&
+\frac{3}{4}\,G(\lambda ;0,y)\,G(\lambda ,\lambda ;x,y)\,H(0;x_0)\\&
-\left( \frac{3}{8} \right) \,G(\lambda ;0,y)\,G(\lambda ,\lambda ;x,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) }{4}\,G(\lambda ;0,y)\,G(\lambda ,x\lambda ;x,y)\,H(0;x_0)\\&
+\frac{3\,\left( -1 + y \right) }{8}\,G(\lambda ;0,y)\,G(\lambda ,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-1 + x + y}{2\,\lambda}\,G(\lambda ;0,y)\,G(x_0,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;0,y)\,G(x_0,\lambda ;x,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(\lambda ;0,y)\,G(x_0,x\lambda ;x,y)\,H(0;x_0)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;0,y)\,G(x_0,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-1 + x + y}{2\,\lambda}\,G(\lambda ;0,y)\,G(x_1,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;0,y)\,G(x_1,\lambda ;x,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(\lambda ;0,y)\,G(x_1,x\lambda ;x,y)\,H(0;x_0)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;0,y)\,G(x_1,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{4\,\lambda}\,G(\lambda ;0,y)\,G(x\lambda ,0;x,y)\,H(0;x_0)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{8\,\lambda}\,G(\lambda ;0,y)\,G(x\lambda ,0;x,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) }{4}\,G(\lambda ;0,y)\,G(x\lambda ,\lambda ;x,y)\,H(0;x_0)\\&
+\frac{3\,\left( -1 + y \right) }{8}\,G(\lambda ;0,y)\,G(x\lambda ,\lambda ;x,y)\,H(0;y)\\&
+\frac{3\,{\left( -1 + y \right) }^2}{4}\,G(\lambda ;0,y)\,G(x\lambda ,x\lambda ;x,y)\,H(0;x_0)\\&
+\frac{-3\,{\left( -1 + y \right) }^2}{8}\,G(\lambda ;0,y)\,G(x\lambda ,x\lambda ;x,y)\,H(0;y)\\&
+\frac{5\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;x,y)\,G(x\lambda ;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(\lambda ;x,y)\,G(x\lambda ;0,y)\,H(0,0;y)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;x,y)\,G(x\lambda ;0,y)\,H(1,0;y)\\&
+\frac{-1 + x + y}{8\,\lambda}\,G(\lambda ;x,y)\,G(0,0;0,y)\,H(0;y)\\&
+\frac{-1 + x + y}{2\,\lambda}\,G(\lambda ;x,y)\,G(0,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-3\,\left( -1 + x + y \right) }{8\,\lambda}\,G(\lambda ;x,y)\,G(0,\lambda ;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{8\,\lambda}\,G(\lambda ;x,y)\,G(0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{3\,\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;x,y)\,G(\lambda ,0;0,y)\,H(0;x_0)\\&
+\frac{-1 + x + y}{8\,\lambda}\,G(\lambda ;x,y)\,G(\lambda ,0;0,y)\,H(0;y)\\&
+\frac{-\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;x,y)\,G(\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-1 + x + y}{8\,\lambda}\,G(\lambda ;x,y)\,G(\lambda ,\lambda ;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{4\,\lambda}\,G(\lambda ;x,y)\,G(\lambda ,x\lambda ;0,y)\,H(0;x_0)\\&
+\frac{3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{8\,\lambda}\,G(\lambda ;x,y)\,G(\lambda ,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-1 + x + y}{2\,\lambda}\,G(\lambda ;x,y)\,G(x_0,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;x,y)\,G(x_0,\lambda ;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{4\,\lambda}\,G(\lambda ;x,y)\,G(x_0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-1 + x + y}{2\,\lambda}\,G(\lambda ;x,y)\,G(x_1,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-\left( -1 + x + y \right) }{4\,\lambda}\,G(\lambda ;x,y)\,G(x_1,\lambda ;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{4\,\lambda}\,G(\lambda ;x,y)\,G(x_1,x\lambda ;0,y)\,H(0;y)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{8\,\lambda}\,G(\lambda ;x,y)\,G(x\lambda ,0;0,y)\,H(0;y)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{2\,\lambda}\,G(\lambda ;x,y)\,G(x\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{8\,\lambda}\,G(\lambda ;x,y)\,G(x\lambda ,\lambda ;0,y)\,H(0;y)\\&
+\frac{-\left( {\left( -1 + y \right) }^2\,\left( -1 + x + y \right)  \right) }{8\,\lambda}\,G(\lambda ;x,y)\,G(x\lambda ,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-5\,{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ;0,y)\,G(x\lambda ;x,y)\,H(0;y)\\&
+\frac{{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{2\,\lambda}\,G(x\lambda ;0,y)\,G(x\lambda ;x,y)\,H(0,0;y)\\&
+\frac{-\left( {\left( -1 + y \right) }^2\,\left( -1 + x + y \right)  \right) }{4\,\lambda}\,G(x\lambda ;0,y)\,G(x\lambda ;x,y)\,H(1,0;y)\\&
+\frac{1 - y}{8}\,G(x\lambda ;0,y)\,G(0,0;x,y)\,H(0;y)\\&
+\frac{-1 + y}{2}\,G(x\lambda ;0,y)\,G(0,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-1 + y}{4}\,G(x\lambda ;0,y)\,G(0,\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{8\,\lambda}\,G(x\lambda ;0,y)\,G(0,\lambda ;x,y)\,H(0;y)\\&
+\frac{3\,{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{8\,\lambda}\,G(x\lambda ;0,y)\,G(0,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-1 + y}{2}\,G(x\lambda ;0,y)\,G(\lambda ,0;0,y)\,H(0;x_0)\\&
+\frac{-1 + y}{4}\,G(x\lambda ;0,y)\,G(\lambda ,0;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{8\,\lambda}\,G(x\lambda ;0,y)\,G(\lambda ,0;x,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) }{8}\,G(x\lambda ;0,y)\,G(\lambda ,\lambda ;x,y)\,H(0;y)\\&
+\frac{3\,{\left( -1 + y \right) }^2}{8}\,G(x\lambda ;0,y)\,G(\lambda ,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{4\,\lambda}\,G(x\lambda ;0,y)\,G(x_0,\lambda ;x,y)\,H(0;y)\\&
+\frac{{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ;0,y)\,G(x_0,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{4\,\lambda}\,G(x\lambda ;0,y)\,G(x_1,\lambda ;x,y)\,H(0;y)\\&
+\frac{{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ;0,y)\,G(x_1,x\lambda ;x,y)\,H(0;y)\\&
+\frac{{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{8\,\lambda}\,G(x\lambda ;0,y)\,G(x\lambda ,0;x,y)\,H(0;y)\\&
+\frac{3\,{\left( -1 + y \right) }^2}{8}\,G(x\lambda ;0,y)\,G(x\lambda ,\lambda ;x,y)\,H(0;y)\\&
+\frac{-3\,{\left( -1 + y \right) }^3}{8}\,G(x\lambda ;0,y)\,G(x\lambda ,x\lambda ;x,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{8\,\lambda}\,G(x\lambda ;x,y)\,G(0,0;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(x\lambda ;x,y)\,G(0,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{8\,\lambda}\,G(x\lambda ;x,y)\,G(0,\lambda ;0,y)\,H(0;y)\\&
+\frac{{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{8\,\lambda}\,G(x\lambda ;x,y)\,G(0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-3\,\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ;x,y)\,G(\lambda ,0;0,y)\,H(0;x_0)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{8\,\lambda}\,G(x\lambda ;x,y)\,G(\lambda ,0;0,y)\,H(0;y)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ;x,y)\,G(\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{8\,\lambda}\,G(x\lambda ;x,y)\,G(\lambda ,\lambda ;0,y)\,H(0;y)\\&
+\frac{{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ;x,y)\,G(\lambda ,x\lambda ;0,y)\,H(0;x_0)\\&
+\frac{-3\,{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{8\,\lambda}\,G(x\lambda ;x,y)\,G(\lambda ,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(x\lambda ;x,y)\,G(x_0,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ;x,y)\,G(x_0,\lambda ;0,y)\,H(0;y)\\&
+\frac{{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ;x,y)\,G(x_0,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-\left( \left( -1 + y \right) \,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(x\lambda ;x,y)\,G(x_1,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{\left( -1 + y \right) \,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ;x,y)\,G(x_1,\lambda ;0,y)\,H(0;y)\\&
+\frac{{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{4\,\lambda}\,G(x\lambda ;x,y)\,G(x_1,x\lambda ;0,y)\,H(0;y)\\&
+\frac{-\left( {\left( -1 + y \right) }^2\,\left( -1 + x + y \right)  \right) }{8\,\lambda}\,G(x\lambda ;x,y)\,G(x\lambda ,0;0,y)\,H(0;y)\\&
+\frac{-\left( {\left( -1 + y \right) }^2\,\left( -1 + x + y \right)  \right) }{2\,\lambda}\,G(x\lambda ;x,y)\,G(x\lambda ,\lambda ;0,y)\,H(0;x_0)\\&
+\frac{3\,{\left( -1 + y \right) }^2\,\left( -1 + x + y \right) }{8\,\lambda}\,G(x\lambda ;x,y)\,G(x\lambda ,\lambda ;0,y)\,H(0;y)\\&
+\frac{{\left( -1 + y \right) }^3\,\left( -1 + x + y \right) }{8\,\lambda}\,G(x\lambda ;x,y)\,G(x\lambda ,x\lambda ;0,y)\,H(0;y)\\&

